WaSt-3D: Wasserstein-2 Distance for Scene-to-Scene Stylization on 3D Gaussians

While style transfer techniques have been well-developed for 2D image stylization, the extension of these methods to 3D scenes remains relatively unexplored. Existing approaches demonstrate proficiency in transferring colors and textures but often struggle with replicating the geometry of the scenes. In our work, we leverage an explicit Gaussian Splatting (GS) representation and directly match the distributions of Gaussians between style and content scenes using the Earth Mover's Distance (EMD). By employing the entropy-regularized Wasserstein-2 distance, we ensure that the transformation maintains spatial smoothness. Additionally, we decompose the scene stylization problem into smaller chunks to enhance efficiency. This paradigm shift reframes stylization from a pure generative process driven by latent space losses to an explicit matching of distributions between two Gaussian representations. Our method achieves high-resolution 3D stylization by faithfully transferring details from 3D style scenes onto the content scene. Furthermore, WaSt-3D consistently delivers results across diverse content and style scenes without necessitating any training, as it relies solely on optimization-based techniques. See our project page for additional results and source code: $\href{https://compvis.github.io/wast3d/}{https://compvis.github.io/wast3d/}$.

==> figures/fig_arcimboldo_painting.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{images/Arcimboldo.jpg}
    \caption{Painting ``Autumn'' by Guiseppe Arcimboldo.}
    \label{fig:arcimboldo_autumn}
\end{figure}


==> figures/fig_color_as_coord_with_edges.tex <==
% \begin{figure}
%     \centering
%     \subfloat{
%         % \label{ref_label1}
%         \includegraphics{images/img_color_as_coord.png}
%     }
    
%     \subfloat{
%         % \label{ref_label2}
%         \includegraphics{images/img_color_as_coord_with_edges.png}
%     }
%     \caption{Color as coordinates representation. With and without SAM edges optimized into the weights of the gaussians. The reader can see that the content becomes more apparent while image has barely changed.}
%     \label{fig:color_as_coord_with_edges}
% \end{figure}


\begin{figure}%
    \centering
    \subfloat{{\includegraphics[width=.45\linewidth]{images/img_color_as_coord.png} }}
    % \qquad
    \subfloat{{\includegraphics[width=.45\linewidth]{images/img_color_as_coord_with_edges.png} }}
    \caption{Color as coordinates representation. With and without SAM edges optimized into the weights of the gaussians. The reader can see that the content becomes more apparent while image has barely changed.}
    \label{fig:color_as_coord_with_edges}
\end{figure}

==> figures/fig_example1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/hotdog_3_styles.png}
    \caption{Our stylization of the hotdog scene using 3 different style scenes }
    \label{fig:hotdog_3_styles}
\end{figure}

==> figures/fig_example2.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/hotdog_1_style.png}
    \caption{Our stylization of the hotdog scene using 1 style scene.}
    \label{fig:enterhotdog_1_style}
\end{figure}

==> figures/fig_title.tex <==

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/Title_page_drawing.pdf}
    \caption{Our stylization of the hot dog scene using 2 different style scenes. Not high resolution 3D details as depicted in the last column. Our method works by locally solving optimal transort problem between patches of content scene and style scene.}
    \label{fig:title}
\end{figure}

==> tex/background.tex <==
\section{Background}

\subsection{Gaussian splatting representation}
Neural Radiance Fields (NeRFs)~\cite{XXX} have been widely utilized over the past few years since its introduction as the neural network based representation implicitly learns the scene density and view-dependent color. This allows for high-quality novel view synthesis once the NeRF model is optimized from a set of 2D input images. More recently, 3D Gaussian Splatting (3DGS)~\cite{kerbl3Dgaussians} has emerged as a powerful alternative that provides significant advantages in terms of optimization speed and real-time rendering while matching the state-of-the-art quality from NeRF-based approaches. 3DGS achieves this by relying on explicit representation based on 3D Gaussians in contrast to the implicit representation of NeRF. To enable high-quality scene reconstruction, each Gaussian is characterized by a set of learnable parameters such as position $\mathbf{x}$, color $\mathbf{c}$, covariance matrix $\Sigma$ (shape and orientation) and opacity $\alpha$. The rendering equation for a typical point-based approach is defined as:
\begin{equation}
	\label{eq:rendered_color}
	C = \sum_{i \in \mathcal{N}}
	\mathbf{c}_{i}\alpha_i
	\prod_{j=1}^{i-1}(1-\alpha_j).
\end{equation}
Here, $\mathcal{N}$ is the number of ordered points along the ray that are $\alpha$-blended per pixel and $\alpha_i$ is the blending opacity obtained by evaluating the 2D Gaussian projection at the pixel and multiplying it with the global opacity $\alpha$.

